Selecting the Selection

Modern saturation-based Automated Theorem Provers typically implement the superposition calculus for reasoning about first-order logic with or without equality. Practical implementations of this calculus use a variety of literal selections and term orderings to tame the growth of the search space and help steer proof search. This paper introduces the notion of lookahead selection that estimates (looks ahead) the effect on the search space of selecting a literal. There is also a case made for the use of incomplete selection functions that attempt to restrict the search space instead of satisfying some completeness criteria. Experimental evaluation in the \Vampire\ theorem prover shows that both lookahead selection and incomplete selection significantly contribute to solving hard problems unsolvable by other methods.

==> flipping.tex <==
% !TEX root = main.tex

\section{Predicate Polarity Flipping} \label{sec:flipping}

The completeness condition (page \pageref{cond:complete}) is not symmetrical
with respect to predicate polarity. It says that it is sufficient
to select a single negative literal, but if we cannot do that
we need to select all the maximal literals in a clause.
This leads to the natural question whether there could be 
a complete version of the superposition calculus 
in which the role of negative and positive literals is exchanged.

We can justify a positive answer to this question
by considering a transformation of the input problem
in which we consistently flip the polarity of every predicate (except for equality)
by changing the corresponding literals from positive to negative and vice versa.
This is easily seen to be satisfiability preserving 
and essentially flips ``the meaning'' of what was positive and negative
in the original problem. We cannot do this with equality literals,
because of the special semantics of the equality predicate.\footnote{
We could do it if equality was explicitly axiomatized in the problem, 
but then we could not use superposition for efficient equality reasoning.
% and would need to fall back to resolution.
}

% Why can it not apply to equality? ... this is one of the reasons we do not use equality predicate only

% need to select either a negative equality literal, a positive non-equality literal
% or all maximal positive equality literals and negative non-equality literals

In \Vampire{}, there is no initial transformation of the input.
Instead, the option to perform \emph{predicate polarity flipping}
is implicitly realized within the code of the selection strategies,
which does not directly query polarity of literals, but may perform a flip depending on the option's value.
Also the code implementing the factoring inference is affected, 
as we want to factor on ``positive'' literals only.
%
We report on the effect of literal polarity flipping in the experimental section.\footnote{
Once could, in principle, also consider flipping the polarity of each predicate
separately. However, this would increase the space of possible strategies by a factor of $2^n$,
where $n$ is the number of predicate symbols, with no obvious simple answer to which of these strategies should be
preferred.}


==> related.tex <==
% !TEX root = main.tex

\section{Related work}
\label{sec:related}

\MS{If we find it is worth mentioning.}

In E: ``Literal selection is controlled by one of about 100 hard-coded selection strategies. In automatic mode, the prover with [sic!] pick one of them without user intervention.'' (see \url{http://wwwlehre.dhbw-stuttgart.de/~sschulz/E/Technology.html}) However, they are alwayslete.

\url{http://wwwlehre.dhbw-stuttgart.de/~sschulz/WORK/E_DOWNLOAD/V_1.9/eprover.pdf} describes selections which can select positive literals provided they select a negative one. So E is in some sense non-standard in this respect as well.
``Each of the strategies that do actually select negative literals has a corresponding
counterpart starting with P that additionally allows paramodulation into maximal positive literals''

Is SPASS: The user can name a subset of predicates such that one negative literal with that predicate is always selected (if present).
They have: SELECTOFF, SELECTIFSEVERALMAXIMAL, SELECTALWAYS, SELECTFROMLIST. Look at \verb|clause_SelectLiteral| in \verb|clause.c|. It is confusing. If it is not from the user and selection still applies, SPASS will go for a single literal with maximal weight (among the negative ones). So the difference between SELECTIFSEVERALMAXIMAL, SELECTALWAYS is that nothing will be selected with SELECTIFSEVERALMAXIMAL if there is just one maximal. 
